Semantic expressive capacity with bounded memory

We investigate the capacity of mechanisms for compositional semantic parsing to describe relations between sentences and semantic representations. We prove that in order to represent certain relations, mechanisms which are syntactically projective must be able to remember an unbounded number of locations in the semantic representations, where nonprojective mechanisms need not. This is the first result of this kind, and has consequences both for grammar-based and for neural systems.

==> discussion.tex <==
\section{Discussion} \label{sec:discussion}

\begin{itemize}
\item Generative device could be neural network.
\item Theorem with alignments applies to shift-reduce parsers. To
  escape the limitations, need to (a) assume non-projective reduce
  steps (check shift-reduce for TAG; shuffle operations for
  non-projective transition-based dependency parsers); or (b) assume
  non-compositional ways for building up the semantic representation
  \cite{E17-1051}; or (c) give up alignments (this seems stupid); or
  (d) maybe get a semantic algebra with infinite memory capacity.
\item The string-graph relation we looked at is functional; we didn't
  even need ambiguity to make the semantic construction problem hard
  in terms of memory capacity. Instead, the difficulty comes from
  keeping track of unboundedly many semantic arguments that are close
  to each other but distant from their predicates in the surface
  string.
\end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

